Supervised Community Detection with Line Graph Neural Networks

Traditionally, community detection in graphs can be solved using spectral methods or posterior inference under probabilistic graphical models. Focusing on random graph families such as the stochastic block model, recent research has unified both approaches and identified both statistical and computational detection thresholds in terms of the signal-to-noise ratio. By recasting community detection as a node-wise classification problem on graphs, we can also study it from a learning perspective. We present a novel family of Graph Neural Networks (GNNs) for solving community detection problems in a supervised learning setting. We show that, in a data-driven manner and without access to the underlying generative models, they can match or even surpass the performance of the belief propagation algorithm on binary and multi-class stochastic block models, which is believed to reach the computational threshold. In particular, we propose to augment GNNs with the non-backtracking operator defined on the line graph of edge adjacencies. Our models also achieve good performance on real-world datasets. In addition, we perform the first analysis of the optimization landscape of training linear GNNs for community detection problems, demonstrating that under certain simplifications and assumptions, the loss values at local and global minima are not far apart.

==> sbm.tex <==


 %It was shown in \cite{M} that detection is possible if and only if $(a-b)^2 > 2(a+b)$. These two inequaities give the information theoretic threshold for exact recovery and detection respectively.  In both cases there is a polynomial time algorithm if $a$ and $b$ satisfy the threshold, and impossible to recover/detect the node labels if not. The detection regime 

 %Trimming these, as trick that works in denser regimes do not work here as sometimes it even destroys the gianto component.  The sparse case connectivity is delicate.  SDP also does not work.  spectral algorithm on non-backtraking operator allows problem to reduce back to problem of reconstruction on trees. 
%The Bayes optimal algorithm is Belief Propagation (BP), which apriori requires quadratic complexity in the number of nodes per iteration (can be reduced to linear for constant degree SBM) and takes very long convergence time at the inforamtion theoretic thresholds\cite{Draza} with no guarantees to converge for non-trees.  Furthermore BP requires the parameters of the SBM to be known in order to recover the nodes, or else the parameter need to be learned. 



%BP: O(N〈k〉q2) 


%the informationtheoretic threshold: the point at which Bayesian inference, given full access
% to the posterior distribution, would find an accurate partition.

